Pose-GNN : Camera Pose Estimation System Using Graph Neural Networks

We propose a novel image based localization system using graph neural networks (GNN). The pretrained ResNet50 convolutional neural network (CNN) architecture is used to extract the important features for each image. Following, the extracted features are input to GNN to find the pose of each image by either using the image features as a node in a graph and formulate the pose estimation problem as node pose regression or modelling the image features themselves as a graph and the problem becomes graph pose regression. We do an extensive comparison between the proposed two approaches and the state of the art single image localization methods and show that using GNN leads to enhanced performance for both indoor and outdoor environments.

==> refs.tex <==
@ARTICLE{vanderGeeretal2000,
  author  = {van der Geer, J. and Hanraads, J. A. J. and Lupton, R. A.},
  title   = {The art of writing a scientific article},
  journal = {J. Sci. Commun.}, 
  volume  = {163},
  year    = {2000},
  pages   = {51-59}
}

@BOOK{StrunkWhite1979,
  author  = {Strunk Jr., W. and White, E. B.},
  title   = {The Elements of Style},
  edition = {3rd},
  address = {New York, NY},
  publisher = {Macmillan},
  year    = {1979}
}

@INCOLLECTION{MettamAdams1999,
  author  = {Mettam, G. R. and Adams, L. B.},
  title   = {How to prepare an electronic version of your article},
  editor  = {Jones, B. S. and Smith, R. Z.},
  booktitle = {Introduction to the Electronic Age},
  address = {New York, NY},
  publisher = {E-Publishing Inc.},
  year    = {1999},
  pages   = {281-304}
}

@ARTICLE{vanderGeeretal2000,
  author  = {van der Geer, J. and Hanraads, J. A. J. and Lupton, R. A.},
  title   = {The art of writing a scientific article},
  journal = {J. Sci. Commun.}, 
  volume  = {163},
  year    = {2000},
  pages   = {51-59}
}

@BOOK{StrunkWhite1979,
  author  = {Strunk Jr., W. and White, E. B.},
  title   = {The Elements of Style},
  edition = {3rd},
  address = {New York, NY},
  publisher = {Macmillan},
  year    = {1979}
}

@INCOLLECTION{MettamAdams1999,
  author  = {Mettam, G. R. and Adams, L. B.},
  title   = {How to prepare an electronic version of your article},
  editor  = {Jones, B. S. and Smith, R. Z.},
  booktitle = {Introduction to the Electronic Age},
  address = {New York, NY},
  publisher = {E-Publishing Inc.},
  year    = {1999},
  pages   = {281-304}
}

@ARTICLE{vanderGeeretal2000,
  author  = {van der Geer, J. and Hanraads, J. A. J. and Lupton, R. A.},
  title   = {The art of writing a scientific article},
  journal = {J. Sci. Commun.}, 
  volume  = {163},
  year    = {2000},
  pages   = {51-59}
}

@BOOK{StrunkWhite1979,
  author  = {Strunk Jr., W. and White, E. B.},
  title   = {The Elements of Style},
  edition = {3rd},
  address = {New York, NY},
  publisher = {Macmillan},
  year    = {1979}
}

@INCOLLECTION{MettamAdams1999,
  author  = {Mettam, G. R. and Adams, L. B.},
  title   = {How to prepare an electronic version of your article},
  editor  = {Jones, B. S. and Smith, R. Z.},
  booktitle = {Introduction to the Electronic Age},
  address = {New York, NY},
  publisher = {E-Publishing Inc.},
  year    = {1999},
  pages   = {281-304}
}



@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  publisher={MIT Press}
  volume={9},
  pages={1735--1780},
  year={1997}
  
}

@article{graves2005framewise,
  title={Framewise phoneme classification with bidirectional LSTM and other neural network architectures},
  author={Graves, Alex and Schmidhuber, J{\"u}rgen},
  journal={Neural Networks},
  volume={18},
  number={5-6},
  pages={602--610},
  year={2005},
  publisher={Elsevier}
}

@article{lecun1995convolutional,
  title={Convolutional networks for images, speech, and time series},
  author={LeCun, Yann and Bengio, Yoshua and others},journal={The handbook of brain theory and neural networks},volume={3361},year={1995}}
  
@inproceedings{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097--1105},
  year={2012}
}

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},

title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
pages = {1527--1554},
year = {2006}
}

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},

title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
pages = {1527--1554},
year = {2006}
}

@article{zhang2016understanding,
  title={Understanding deep learning requires rethinking generalization},
  author={Zhang, Chiyuan and Bengio, Samy and Hardt, Moritz and Recht, Benjamin and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1611.03530},
  year={2016}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{ioffe2015batch,
  title={Batch normalization: Accelerating deep network training by reducing internal covariate shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  booktitle={International Conference on Machine Learning},
  pages={448--456},
  year={2015}
}

@article{bay2008speeded,
  title={Speeded-up robust features {(SURF)}},
  author={Bay, Herbert and Ess, Andreas and Tuytelaars, Tinne and Van Gool, Luc},
  journal={Computer vision and image understanding},
  publisher={Elsevier}
  volume={110},
  pages={346--359},
  year={2008},
  
}

@inproceedings{du2009face,
  title={Face recognition using {SURF} features},
  author={Du, Geng and Su, Fei and Cai, Anni},
  booktitle={Proc. of SPIE Vol},
  volume={7496},
  pages={749628--1},
  year={2009}
}

@inproceedings{engelhard2011real,
  title={Real-time 3D visual {SLAM} with a hand-held RGB-D camera},
  author={Engelhard, Nikolas and Endres, Felix and Hess, J{\"u}rgen and Sturm, J{\"u}rgen and Burgard, Wolfram},
  booktitle={Proc. of the RGB-D Workshop on 3D Perception in Robotics at the European Robotics Forum, Vasteras, Sweden},
  volume={180},
  pages={1--15},
  year={2011}
}

@inproceedings{chincha2011finding,
  title={Finding objects for blind people based on {SURF} features},
  author={Chincha, Ricardo and Tian, YingLi},
  booktitle={IEEE International Conference on Bioinformatics and Biomedicine Workshops (BIBMW)},
  pages={526--527},
  year={2011}

}

@inproceedings{rublee2011orb,
  title={{ORB}: An efficient alternative to {SIFT} or {SURF}},
  author={Rublee, Ethan and Rabaud, Vincent and Konolige, Kurt and Bradski, Gary},
  booktitle={IEEE international conference on Computer Vision (ICCV)},
  pages={2564--2571},
  year={2011}
}

@inproceedings{alahi2012freak,
  title={Freak: Fast retina keypoint},
  author={Alahi, Alexandre and Ortiz, Raphael and Vandergheynst, Pierre},
  booktitle={IEEE conference on Computer vision and pattern recognition (CVPR)},
  pages={510--517},
    year={2012}

}

@book{bradski2008learning,
  title={Learning OpenCV: Computer vision with the OpenCV library},
  author={Bradski, Gary and Kaehler, Adrian},
 
  publisher={" O'Reilly Media, Inc."},
   year={2008},
}

@inproceedings{glocker2013real,
  title={Real-time {RGB-D} camera relocalization},
  author={Glocker, Ben and Izadi, Shahram and Shotton, Jamie and Criminisi, Antonio},
  booktitle={IEEE International Symposium on Mixed and Augmented Reality (ISMAR) },
  pages={173--179},
  year={2013}

}

@inproceedings{lai2014unsupervised,
  title={Unsupervised feature learning for 3d scene labeling},
  author={Lai, Kevin and Bo, Liefeng and Fox, Dieter},
  booktitle={IEEE International Conference on Robotics and Automation (ICRA) },
  pages={3050--3057},
  year={2014}

}

@inproceedings{kendall2015posenet,
  title={Posenet: A convolutional network for real-time 6-dof camera relocalization},
  author={Kendall, Alex and Grimes, Matthew and Cipolla, Roberto},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2938--2946},
  year={2015}
}
@article{melekhov2017image,
  title={Image-based Localization using Hourglass Networks},
  author={Melekhov, Iaroslav and Ylioinas, Juha and Kannala, Juho and Rahtu, Esa},
  journal={arXiv preprint arXiv:1703.07971},
  year={2017}
}



@article{hazirbasimage,
  title={Image-based localization using lstms for structured feature correlation},
  author={Walch, Florian and Hazirbas, Caner and Leal-Taixe, Laura and Sattler, Torsten and Hilsenbeck, Sebastian and Cremers, Daniel},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={627--637},
  year={2017}
}
@article{lowe2004distinctive,
  title={Distinctive image features from scale-invariant keypoints},
  author={Lowe, David G},
  journal={International journal of computer vision},
   publisher={Springer}
  volume={60},
  pages={91--110},
  year={2004},
 
}

@article{srivastava2014dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting.},
  author={Srivastava, Nitish and Hinton, Geoffrey E and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={Journal of machine learning research},
  volume={15},
  pages={1929--1958},
  year={2014}
}
@book{xu2016gps,
  title={{GPS}: theory, algorithms and applications},
  author={Xu, Guochang and Xu, Yan},

  publisher={Springer},
    year={2016},
}

@article{durrant2006simultaneous,
  title={Simultaneous localization and mapping: part I},
  author={Durrant-Whyte, Hugh and Bailey, Tim},
  journal={IEEE robotics \& automation magazine},
  publisher={IEEE},
  volume={13},
  pages={99--110},
  year={2006},
  
}

@inproceedings{sattler2015hyperpoints,
  title={Hyperpoints and fine vocabularies for large-scale location recognition},
  author={Sattler, Torsten and Havlena, Michal and Radenovic, Filip and Schindler, Konrad and Pollefeys, Marc},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2102--2110},
  year={2015}
}

@inproceedings{sattler2011fast,
  title={Fast image-based localization using direct 2d-to-3d matching},
  author={Sattler, Torsten and Leibe, Bastian and Kobbelt, Leif},
  booktitle={IEEE International Conference on Computer Vision (ICCV),  },
  pages={667--674},
   year={2011},

}


@article{sattler2017efficient,
  title={Efficient \& effective prioritized matching for large-scale image-based localization},
  author={Torsten, Sattler and Leibe, Bastian and Kobbelt, Leif},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={39},
  pages={1744--1756},
  year={2017},

}

@inproceedings{oquab2014learning,
  title={Learning and transferring mid-level image representations using convolutional neural networks},
  author={Oquab, Maxime and Bottou, Leon and Laptev, Ivan and Sivic, Josef},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1717--1724},
  year={2014}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}


@article{schmidhuber1997long,
  title={Long short-term memory},
  author={Schmidhuber, J{\"u}rgen and Hochreiter, Sepp},
  journal={Neural Comput},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}


@book{forsyth2011computer,
  title={Computer vision: a modern approach},
  author={Forsyth, David and Ponce, Jean},
   publisher={Upper Saddle River, NJ; London: Prentice Hall},
  year={2011},
 
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{kalantidis2009visual,
  title={Visual image retrieval and localization},
  author={Kalantidis, Yannis and Tolias, Giorgos and Spyrou, Evaggelos and Mylonas, Phivos and Avrithis, Yannis},
  booktitle={7th International Workshop on Content-Based Multimedia Indexing, Greece},
  year={2009}
}

@article{bayraktar2017analysis,
  title={Analysis of feature detector and descriptor combinations with a localization experiment for various performance metrics},
  author={Bayraktar, Ertugrul and Boyraz, Pinar},
  journal={arXiv preprint arXiv:1710.06232},
  year={2017}
}
@article{dollar2014fast,
  title={Fast feature pyramids for object detection},
  author={Doll{\'a}r, Piotr and Appel, Ron and Belongie, Serge and Perona, Pietro},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={36},
  pages={1532--1545},
  year={2014},

}


@inproceedings{calonder2010brief,
  title={Brief: Binary robust independent elementary features},
  author={Calonder, Michael and Lepetit, Vincent and Strecha, Christoph and Fua, Pascal},
  booktitle={European conference on computer vision},
  organization={Springer},
  pages={778--792},
  year={2010},
  
}

@article{parkinson1996gps,
  title={{GPS} error analysis},
  author={Parkinson, Bradford W},
  journal={Global Positioning System: Theory and Applications.},
  volume={1},
  pages={469--483},
  year={1996}
}

@article{miura2015gps,
  title={{GPS} error correction with pseudorange evaluation using three-dimensional maps},
  author={Miura, Shunsuke and Hsu, Li-Ta and Chen, Feiyu and Kamijo, Shunsuke},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={16},
  pages={3104--3115},
  year={2015},

}


@article{liu2007survey,
  title={Survey of wireless indoor positioning techniques and systems},
  author={Liu, Hui and Darabi, Houshang and Banerjee, Pat and Liu, Jing},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part C (Applications and Reviews)},
  volume={37},
  pages={1067--1080},
  year={2007},

}

@article{cadena2016past,
  title={Past, present, and future of simultaneous localization and mapping: Toward the robust-perception age},
  author={Cadena, Cesar and Carlone, Luca and Carrillo, Henry and Latif, Yasir and Scaramuzza, Davide and Neira, Jos{\'e} and Reid, Ian and Leonard, John J},
  journal={IEEE Transactions on Robotics},
  volume={32},
  pages={1309--1332},
  year={2016},

}

@article{chen1997haar,
  title={Haar wavelet method for solving lumped and distributed-parameter systems},
  author={Chen, CF and Hsiao, CH},
  journal={IEEE Proceedings-Control Theory and Applications},
  publisher={IET},
  volume={144},
  pages={87--94},
  year={1997},
  
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{su2015multi,
  title={Multi-view convolutional neural networks for 3d shape recognition},
  author={Su, Hang and Maji, Subhransu and Kalogerakis, Evangelos and Learned-Miller, Erik},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={945--953},
  year={2015}
}

@inproceedings{chen2016invariant,
  title={Invariant descriptor learning using a Siamese convolutional neural network},
  author={Chen, Lin and Rottensteiner, Franz and Heipke, Christian},
  booktitle={XXIII ISPRS Congress, Commission III 3 (2016), Nr. 3},
 
 
  organization={G{\"o}ttingen: Copernicus GmbH},
   volume={3},
   pages={11--18},
  year={2016},
}


@inproceedings{simo2015discriminative,
  title={Discriminative learning of deep convolutional feature point descriptors},
  author={Simo-Serra, Edgar and Trulls, Eduard and Ferraz, Luis and Kokkinos, Iasonas and Fua, Pascal and Moreno-Noguer, Francesc},
  booktitle={ IEEE International Conference on Computer Vision (ICCV)},
  pages={118--126},
  year={2016}

}


@inproceedings{lin2016learning,
  title={Learning compact binary descriptors with unsupervised deep neural networks},
  author={Lin, Kevin and Lu, Jiwen and Chen, Chu-Song and Zhou, Jie},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1183--1192},
  year={2016}
}


@book{hertz2018introduction,
  title={Introduction to the theory of neural computation},
  author={Hertz, John A},
  publisher={CRC Press},
  year={2018}
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{zagoruyko2015learning,
  title={Learning to compare image patches via convolutional neural networks},
  author={Zagoruyko, Sergey and Komodakis, Nikos},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={4353--4361},
  year={2015}

}

@article{fuentes2015visual,
  title={Visual simultaneous localization and mapping: a survey},
  author={Fuentes-Pacheco, Jorge and Ruiz-Ascencio, Jos{\'e} and Rend{\'o}n-Mancha, Juan Manuel},
  journal={Artificial Intelligence Review},
 
  publisher={Springer},
   volume={43},
   pages={55--81},
  
}

@article{mur2015orb,
  title={{ORB-SLAM}: a versatile and accurate monocular SLAM system},
  author={Mur-Artal, Raul and Montiel, Jose Maria Martinez and Tardos, Juan D},
  journal={IEEE Transactions on Robotics},
  volume={31},
  pages={1147--1163},
  year={2015},

}

@article{mur2017orb,
  title={Orb-slam2: An open-source slam system for monocular, stereo, and rgb-d cameras},
  author={Mur-Artal, Raul and Tard{\'o}s, Juan D},
  journal={IEEE Transactions on Robotics},
  volume={33},
  pages={1255--1262},
  year={2017},

}

@article{mur2017orb,
  title={Orb-slam2: An open-source slam system for monocular, stereo, and rgb-d cameras},
  author={Mur-Artal, Raul and Tard{\'o}s, Juan D},
  journal={IEEE Transactions on Robotics},
  volume={33},
  pages={1255--1262},
  year={2017},

}

@book{hartley2003multiple,
  title={Multiple view geometry in computer vision},
  author={Hartley, Richard and Zisserman, Andrew},
  publisher={Cambridge university press},
  year={2003}
}

@inproceedings{engel2014lsd,
  title={{LSD-SLAM}: Large-scale direct monocular {SLAM}},
  author={Engel, Jakob and Sch{\"o}ps, Thomas and Cremers, Daniel},
  booktitle={European Conference on Computer Vision},
   organization={Springer},
  pages={834--849},
  year={2014}
 
}

@InProceedings{ sturm12iros,
	author = {J. Sturm and N. Engelhard and F. Endres and W. Burgard and D. Cremers},
	title = "A Benchmark for the Evaluation of {RGB-D SLAM} Systems",
	booktitle = "Proc. of the International Conference on Intelligent Robot Systems (IROS)",
	year = "2012",
	month= "Oct.",
}

InProceedings{ handaICRA2014,
author = {A. Handa and T. Whelan and J.B. McDonald and A.J. Davison},
title = {A Benchmark for {RGB-D} Visual Odometry, {3D} Reconstruction and {SLAM}},
booktitle = {IEEE Intl. Conf. on Robotics and Automation, ICRA},
address = {Hong Kong, China},
month = {May},
year = {2014}
}

@inproceedings{handa2014benchmark,
  title={A benchmark for {RGB-D} visual odometry, {3D} reconstruction and {SLAM}},
  author={Handa, Ankur and Whelan, Thomas and McDonald, John and Davison, Andrew J},
  booktitle={IEEE international conference on Robotics and automation (ICRA) },
  pages={1524--1531},
   year={2014}

}
@inproceedings{szegedy2016rethinking,
  title={Rethinking the inception architecture for computer vision},
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2818--2826},
  year={2016}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew and others},
  organization={Cvpr},
   year={2015}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@book{forsyth2002computer,
  title={Computer vision: a modern approach},
  author={Forsyth, David A and Ponce, Jean},
  
  publisher={Prentice Hall Professional Technical Reference},
  year={2002}
}

@article{hartley1997defense,
  title={In defense of the eight-point algorithm},
  author={Hartley, Richard I},
  journal={IEEE Transactions on pattern analysis and machine intelligence},
  volume={19},
  pages={580--593},
  year={1997},
}

@article{zanella2014internet,
  title={Internet of things for smart cities},
  author={Zanella, Andrea and Bui, Nicola and Castellani, Angelo and Vangelista, Lorenzo and Zorzi, Michele},
  journal={IEEE Internet of Things journal},
    publisher={IEEE}
  volume={1},
  pages={22--32},
  year={2014},
}

@article{alletto2016indoor,
  title={An indoor location-aware system for an IoT-based smart museum},
  author={Alletto, Stefano and Cucchiara, Rita and Del Fiore, Giuseppe and Mainetti, Luca and Mighali, Vincenzo and Patrono, Luigi and Serra, Giuseppe},
  journal={IEEE Internet of Things Journal},
      publisher={IEEE},

  volume={3},
  pages={244--253},
  year={2016},
}

@article{ma2018foglight,
  title={Foglight: Visible Light-Enabled Indoor Localization System for Low-Power IoT Devices},
  author={Ma, Shang and Liu, Qiong and Sheu, Phillip C-Y},
  journal={IEEE Internet of Things Journal},
    publisher={IEEE}
  volume={5},
  pages={175--185},
  year={2018},

}
@inproceedings{rohrig2009indoor,
  title={Indoor location tracking in non-line-of-sight environments using a IEEE 802.15. 4a wireless network},
  author={R{\"o}hrig, Christof and M{\"u}ller, Marcel},
  booktitle={International Conference on Intelligent Robots and Systems},
   organization={IEEE}
  pages={552--557},
  year={2009},
 
}


@inproceedings{lymberopoulos2015realistic,
  title={A realistic evaluation and comparison of indoor location technologies: Experiences and lessons learned},
  author={Lymberopoulos, Dimitrios and Liu, Jie and Yang, Xue and Choudhury, Romit Roy and Handziski, Vlado and Sen, Souvik},
  booktitle={Proceedings of the 14th international conference on information processing in sensor networks},
  pages={178--189},
  year={2015},
  organization={ACM}
}

@article{alletto2016indoor,
  title={An indoor location-aware system for an IoT-based smart museum},
  author={Alletto, Stefano and Cucchiara, Rita and Del Fiore, Giuseppe and Mainetti, Luca and Mighali, Vincenzo and Patrono, Luigi and Serra, Giuseppe},
  journal={IEEE Internet of Things Journal},
    publisher={IEEE},
  volume={3},
  pages={244--253},
  year={2016},

}

@article{mohammadi2018semisupervised,
  title={Semisupervised deep reinforcement learning in support of IoT and smart city services},
  author={Mohammadi, Mehdi and Al-Fuqaha, Ala and Guizani, Mohsen and Oh, Jun-Seok},
  journal={IEEE Internet of Things Journal},
   publisher={IEEE},
  volume={5},
  pages={624--635},
  year={2018}
 
}

@article{klepeis2001national,
  title={The National Human Activity Pattern Survey (NHAPS): a resource for assessing exposure to environmental pollutants},
  author={Klepeis, Neil E and Nelson, William C and Ott, Wayne R and Robinson, John P and Tsang, Andy M and Switzer, Paul and Behar, Joseph V and Hern, Stephen C and Engelmann, William H},
  journal={Journal of Exposure Science and Environmental Epidemiology},
    publisher={Nature Publishing Group}
  volume={11},
  pages={231},
  year={2001},

}


@inproceedings{kendall2017geometric,
  title={Geometric loss functions for camera pose regression with deep learning},
  author={Kendall, Alex and Cipolla, Roberto},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5974--5983},
  year={2017}
}


@inproceedings{kendall2016modelling,
  title={Modelling uncertainty in deep learning for camera relocalization},
  author={Kendall, Alex and Cipolla, Roberto},
  booktitle={2016 IEEE international conference on Robotics and Automation (ICRA)},
  pages={4762--4769},
  year={2016},
  organization={IEEE}
}

@inproceedings{cai2018hybrid,
  title={A Hybrid Probabilistic Model for Camera Relocalization},
  author={Cai, Ming and Shen, Chunhua and Reid, Ian},
  booktitle={British Machine Vision Conference},
  year={2018}
}

@inproceedings{wu2017delving,
  title={Delving deeper into convolutional neural networks for camera relocalization},
  author={Wu, Jian and Ma, Liwei and Hu, Xiaolin},
  booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={5644--5651},
  year={2017},
  organization={IEEE}
}


@article{canziani2016analysis,
  title={An analysis of deep neural network models for practical applications},
  author={Canziani, Alfredo and Paszke, Adam and Culurciello, Eugenio},
  journal={arXiv preprint arXiv:1605.07678},
  year={2016}
}

@article{yassin2016recent,
  title={Recent advances in indoor localization: A survey on theoretical approaches and applications},
  author={Yassin, Ali and Nasser, Youssef and Awad, Mariette and Al-Dubai, Ahmed and Liu, Ran and Yuen, Chau and Raulefs, Ronald and Aboutanios, Elias},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={19},
  number={2},
  pages={1327--1346},
  year={2016},
  publisher={IEEE}
}


@inproceedings{kendall2017geometric,
  title={Geometric loss functions for camera pose regression with deep learning},
  author={Kendall, Alex and Cipolla, Roberto},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5974--5983},
  year={2018}
}

@inproceedings{wu2017delving,
  title={Delving deeper into convolutional neural networks for camera relocalization},
  author={Wu, Jian and Ma, Liwei and Hu, Xiaolin},
  booktitle={2017 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={5644--5651},
  year={2017},
  organization={IEEE}
}

@article{fuentes2015visual,
  title={Visual simultaneous localization and mapping: a survey},
  author={Fuentes-Pacheco, Jorge and Ruiz-Ascencio, Jos{\'e} and Rend{\'o}n-Mancha, Juan Manuel},
  journal={Artificial Intelligence Review},
  volume={43},
  number={1},
  pages={55--81},
  year={2015},
  publisher={Springer}
}
@inproceedings{triggs1999bundle,
  title={Bundle adjustment—a modern synthesis},
  author={Triggs, Bill and McLauchlan, Philip F and Hartley, Richard I and Fitzgibbon, Andrew W},
  booktitle={International workshop on vision algorithms},
  pages={298--372},
  year={1999},
  organization={Springer}
}

@article{ullman1979interpretation,
  title={The interpretation of structure from motion},
  author={Ullman, Shimon},
  journal={Proceedings of the Royal Society of London. Series B. Biological Sciences},
  volume={203},
  number={1153},
  pages={405--426},
  year={1979},
  publisher={The Royal Society London}
}

@inproceedings{schonberger2016structure,
  title={Structure-from-motion revisited},
  author={Schonberger, Johannes L and Frahm, Jan-Michael},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4104--4113},
  year={2016}
}

@article{nister2004efficient,
  title={An efficient solution to the five-point relative pose problem},
  author={Nist{\'e}r, David},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={26},
  number={6},
  pages={0756--777},
  year={2004},
  publisher={IEEE Computer Society}
}

@article{derpanis2010overview,
  title={Overview of the RANSAC Algorithm},
  author={Derpanis, Konstantinos G},
  journal={Image Rochester NY},
  volume={4},
  number={1},
  pages={2--3},
  year={2010}
}

@inproceedings{brachmann2017dsac,
  title={DSAC-differentiable RANSAC for camera localization},
  author={Brachmann, Eric and Krull, Alexander and Nowozin, Sebastian and Shotton, Jamie and Michel, Frank and Gumhold, Stefan and Rother, Carsten},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6684--6692},
  year={2017}
}

@inproceedings{taira2018inloc,
  title={InLoc: Indoor visual localization with dense matching and view synthesis},
  author={Taira, Hajime and Okutomi, Masatoshi and Sattler, Torsten and Cimpoi, Mircea and Pollefeys, Marc and Sivic, Josef and Pajdla, Tomas and Torii, Akihiko},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7199--7209},
  year={2018}
}

@inproceedings{sattler2012image,
  title={Image Retrieval for Image-Based Localization Revisited.},
  author={Sattler, Torsten and Weyand, Tobias and Leibe, Bastian and Kobbelt, Leif},
  booktitle={BMVC},
  volume={1},
  number={2},
  pages={4},
  year={2012}
}

@inproceedings{sattler2015hyperpoints,
  title={Hyperpoints and fine vocabularies for large-scale location recognition},
  author={Sattler, Torsten and Havlena, Michal and Radenovic, Filip and Schindler, Konrad and Pollefeys, Marc},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2102--2110},
  year={2015}
}


@INPROCEEDINGS{SURFCNN,
author={A. M. {Elmoogy} and X. {Dong} and T. {Lu} and R. {Westendorp} and K. {Reddy}},
booktitle={2019 IEEE Pacific Rim Conference on Communications, Computers and Signal Processing (PACRIM)},
title={SurfCNN: A descriptor enhanced convolutional neural network},
year={2019},
volume={},
number={},
pages={1-5},
keywords={CNN;SURF;localization},
doi={10.1109/PACRIM47961.2019.8985026},
ISSN={2325-0445},
month={Aug},}

@article{elmoogy2020surfcnn,
  title={SurfCNN: A Descriptor Accelerated Convolutional Neural Network for Image-Based Indoor Localization},
  author={Elmoogy, Ahmed M and Dong, Xiaodai and Lu, Tao and Westendorp, Robert and Tarimala, Kishore Reddy},
  journal={IEEE Access},
  volume={8},
  pages={59750--59759},
  year={2020},
  publisher={IEEE}
}

@article{SURFLSTM,
author={A. M. {Elmoogy} and X. {Dong} and T. {Lu} and R. {Westendorp} and K. {Reddy}},
booktitle={The 2020 IEEE 92nd Vehicular Technology Conference: VTC2020-Fall},
title={SURF-LSTM: A Descriptor Enhanced Recurrent Neural Network For Indoor Localization},
month={Oct},
year={2020},}

@article{iyer2018geometric,
  title={Geometric Consistency for Self-Supervised End-to-End Visual Odometry},
  author={Iyer, Ganesh and Murthy, J Krishna and Gunshi Gupta, K and Paull, Liam},
  journal={arXiv preprint arXiv:1804.03789},
  year={2018}
}



@article{howard2017mobilenets,
  title={Mobilenets: Efficient convolutional neural networks for mobile vision applications},
  author={Howard, Andrew G and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
  journal={arXiv preprint arXiv:1704.04861},
  year={2017}
}


@inproceedings{cimarelli2019faster,
  title={Faster Visual-Based Localization with Mobile-PoseNet},
  author={Cimarelli, Claudio and Cazzato, Dario and Olivares-Mendez, Miguel A and Voos, Holger},
  booktitle={International Conference on Computer Analysis of Images and Patterns},
  pages={219--230},
  year={2019},
  organization={Springer}
}

@inproceedings{cimarelli2019faster,
  title={Faster Visual-Based Localization with Mobile-PoseNet},
  author={Cimarelli, Claudio and Cazzato, Dario and Olivares-Mendez, Miguel A and Voos, Holger},
  booktitle={International Conference on Computer Analysis of Images and Patterns},
  pages={219--230},
  year={2019},
  organization={Springer}
}


@article{zanella2014internet,
  title={Internet of things for smart cities},
  author={Zanella, Andrea and Bui, Nicola and Castellani, Angelo and Vangelista, Lorenzo and Zorzi, Michele},
  journal={IEEE Internet of Things journal},
  volume={1},
  number={1},
  pages={22--32},
  year={2014},
  publisher={IEEE}
}

@article{khelifi2019survey,
  title={A survey of localization systems in internet of things},
  author={Khelifi, Fekher and Bradai, Abbas and Benslimane, Abderrahim and Rawat, Priyanka and Atri, Mohamed},
  journal={Mobile Networks and Applications},
  volume={24},
  number={3},
  pages={761--785},
  year={2019},
  publisher={Springer}
}

@article{hoang2018soft,
  title={A soft range limited k-nearest neighbors algorithm for indoor localization enhancement},
  author={Hoang, Minh Tu and Zhu, Yizhou and Yuen, Brosnan and Reese, Tyler and Dong, Xiaodai and Lu, Tao and Westendorp, Robert and Xie, Michael},
  journal={IEEE Sensors Journal},
  volume={18},
  number={24},
  pages={10208--10216},
  year={2018},
  publisher={IEEE}
}

@inproceedings{yin2018pclr,
  title={A PCLR-GIST algorithm for fast image retrieval in visual indoor localization system},
  author={Yin, Xiliang and Ma, Lin and Tan, Xuezhi},
  booktitle={2018 IEEE 87th Vehicular Technology Conference (VTC Spring)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@inproceedings{brachmann2017dsac,
  title={Dsac-differentiable ransac for camera localization},
  author={Brachmann, Eric and Krull, Alexander and Nowozin, Sebastian and Shotton, Jamie and Michel, Frank and Gumhold, Stefan and Rother, Carsten},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6684--6692},
  year={2017}
}

@inproceedings{sattler2019understanding,
  title={Understanding the limitations of cnn-based absolute camera pose regression},
  author={Sattler, Torsten and Zhou, Qunjie and Pollefeys, Marc and Leal-Taixe, Laura},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3302--3312},
  year={2019}
}
@article{choi1997performance,
  title={Performance evaluation of RANSAC family},
  author={Choi, Sunglok and Kim, Taemin and Yu, Wonpil},
  journal={Journal of Computer Vision},
  volume={24},
  number={3},
  pages={271--300},
  year={1997}
}

@book{goodfellow2016deep,
  title={Deep learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT press}
}


@article{sze2017efficient,
  title={Efficient processing of deep neural networks: A tutorial and survey},
  author={Sze, Vivienne and Chen, Yu-Hsin and Yang, Tien-Ju and Emer, Joel S},
  journal={Proceedings of the IEEE},
  volume={105},
  number={12},
  pages={2295--2329},
  year={2017},
  publisher={Ieee}
}
@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}

@article{zhou2016places,
  title={Places: An image database for deep scene understanding},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Torralba, Antonio and Oliva, Aude},
  journal={arXiv preprint arXiv:1610.02055},
  year={2016}
}

@inproceedings{song2010feature,
  title={Feature selection using principal component analysis},
  author={Song, Fengxi and Guo, Zhongwei and Mei, Dayong},
  booktitle={2010 international conference on system science, engineering design and manufacturing informatization},
  volume={1},
  pages={27--30},
  year={2010},
  organization={IEEE}
}



@inproceedings{clark2017vidloc,
  title={Vidloc: A deep spatio-temporal model for 6-dof video-clip relocalization},
  author={Clark, Ronald and Wang, Sen and Markham, Andrew and Trigoni, Niki and Wen, Hongkai},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6856--6864},
  year={2017}
}





@article{chen2018rise,
  title={The rise of deep learning in drug discovery},
  author={Chen, Hongming and Engkvist, Ola and Wang, Yinhai and Olivecrona, Marcus and Blaschke, Thomas},
  journal={Drug discovery today},
  volume={23},
  number={6},
  pages={1241--1250},
  year={2018},
  publisher={Elsevier}
}



@article{wu2020comprehensive,
  title={A comprehensive survey on graph neural networks},
  author={Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Philip, S Yu},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2020},
  publisher={IEEE}
}

@inproceedings{shi2019skeleton,
  title={Skeleton-based action recognition with directed graph neural networks},
  author={Shi, Lei and Zhang, Yifan and Cheng, Jian and Lu, Hanqing},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7912--7921},
  year={2019}
}


@article{kipf2016variational,
  title={Variational graph auto-encoders},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1611.07308},
  year={2016}
}


@inproceedings{walch2017image,
  title={Image-based localization using lstms for structured feature correlation},
  author={Walch, Florian and Hazirbas, Caner and Leal-Taixe, Laura and Sattler, Torsten and Hilsenbeck, Sebastian and Cremers, Daniel},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={627--637},
  year={2017}
}

@article{wu2020comprehensive,
  title={A comprehensive survey on graph neural networks},
  author={Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Philip, S Yu},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2020},
  publisher={IEEE}
}

@article{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1609.02907},
  year={2016}
}

@inproceedings{gilmer2017neural,
  title={Neural message passing for quantum chemistry},
  author={Gilmer, Justin and Schoenholz, Samuel S and Riley, Patrick F and Vinyals, Oriol and Dahl, George E},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={1263--1272},
  year={2017},
  organization={JMLR. org}
}

@article{li2015gated,
  title={Gated graph sequence neural networks},
  author={Li, Yujia and Tarlow, Daniel and Brockschmidt, Marc and Zemel, Richard},
  journal={arXiv preprint arXiv:1511.05493},
  year={2015}
}


@inproceedings{monti2017geometric,
  title={Geometric deep learning on graphs and manifolds using mixture model cnns},
  author={Monti, Federico and Boscaini, Davide and Masci, Jonathan and Rodola, Emanuele and Svoboda, Jan and Bronstein, Michael M},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5115--5124},
  year={2017}
}

@article{zhou2018graph,
  title={Graph neural networks: A review of methods and applications},
  author={Zhou, Jie and Cui, Ganqu and Zhang, Zhengyan and Yang, Cheng and Liu, Zhiyuan and Wang, Lifeng and Li, Changcheng and Sun, Maosong},
  journal={arXiv preprint arXiv:1812.08434},
  year={2018}
}

@inproceedings{hamilton2017inductive,
  title={Inductive representation learning on large graphs},
  author={Hamilton, Will and Ying, Zhitao and Leskovec, Jure},
  booktitle={Advances in neural information processing systems},
  pages={1024--1034},
  year={2017}
}

@article{velivckovic2017graph,
  title={Graph attention networks},
  author={Veli{\v{c}}kovi{\'c}, Petar and Cucurull, Guillem and Casanova, Arantxa and Romero, Adriana and Lio, Pietro and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1710.10903},
  year={2017}
}

@inproceedings{morris2019weisfeiler,
  title={Weisfeiler and leman go neural: Higher-order graph neural networks},
  author={Morris, Christopher and Ritzert, Martin and Fey, Matthias and Hamilton, William L and Lenssen, Jan Eric and Rattan, Gaurav and Grohe, Martin},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={4602--4609},
  year={2019}
}

@article{elmoogy2020generalizable,
  title={Generalizable Sequential Camera Pose Learning Using Surf Enhanced 3D CNN},
  author={Elmoogy, Ahmed and Dong, Xiaodai and Lu, Tao and Westendorp, Robert and Reddy, Kishore},
  booktitle={2020 IEEE 92nd Vehicular Technology Conference (VTC2020-Fall)},
  pages={1--6},
  organization={IEEE},
  year ={2020}
}
@article{elmoogy2020surf_lstm,
  title={Surf-lstm: A descriptor enhanced recurrent neural network for indoor localization},
  author={Elmoogy, Ahmed and Dong, Xiaodai and Lu, Tao and Westendorp, Robert and Reddy, Kishore},
  booktitle={2020 IEEE 92nd Vehicular Technology Conference (VTC2020-Fall)},
  pages={1--5},
  year={2020},
  organization={IEEE}
}

@article{elmoogy2020linear,
  title={Linear-PoseNet: A Real-Time Camera Pose Estimation System Using Linear Regression and Principal Component Analysis},
  author={Elmoogy, Ahmed and Dong, Xiaodai and Lu, Tao and Westendorp, Robert and Reddy, Kishore},
  booktitle={2020 IEEE 92nd Vehicular Technology Conference (VTC2020-Fall)},
  pages={1--6},
  organization={IEEE},
  year={2021}
}

@article{dwivedi2020benchmarking,
  title={Benchmarking graph neural networks},
  author={Dwivedi, Vijay Prakash and Joshi, Chaitanya K and Laurent, Thomas and Bengio, Yoshua and Bresson, Xavier},
  journal={arXiv preprint arXiv:2003.00982},
  year={2020}
}

@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}

@article{zhou2016places,
  title={Places: An image database for deep scene understanding},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Torralba, Antonio and Oliva, Aude},
  journal={arXiv preprint arXiv:1610.02055},
  year={2016}
}

@inproceedings{duvenaud2015convolutional,
  title={Convolutional networks on graphs for learning molecular fingerprints},
  author={Duvenaud, David K and Maclaurin, Dougal and Iparraguirre, Jorge and Bombarell, Rafael and Hirzel, Timothy and Aspuru-Guzik, Al{\'a}n and Adams, Ryan P},
  booktitle={Advances in neural information processing systems},
  pages={2224--2232},
  year={2015}
}


@article{peterson2009k,
  title={K-nearest neighbor},
  author={Peterson, Leif E},
  journal={Scholarpedia},
  volume={4},
  number={2},
  pages={1883},
  year={2009}
}

